SFDDM: Single-fold Distillation for Diffusion models

While diffusion models effectively generate remarkable synthetic images, a key limitation is the inference inefficiency, requiring numerous sampling steps. To accelerate inference and maintain high-quality synthesis, teacher-student distillation is applied to compress the diffusion models in a progressive and binary manner by retraining, e.g., reducing the 1024-step model to a 128-step model in 3 folds. In this paper, we propose a single-fold distillation algorithm, SFDDM, which can flexibly compress the teacher diffusion model into a student model of any desired step, based on reparameterization of the intermediate inputs from the teacher model. To train the student diffusion, we minimize not only the output distance but also the distribution of the hidden variables between the teacher and student model. Extensive experiments on four datasets demonstrate that our student model trained by the proposed SFDDM is able to sample high-quality data with steps reduced to as little as approximately 1%, thus, trading off inference time. Our remarkable performance highlights that SFDDM effectively transfers knowledge in single-fold distillation, achieving semantic consistency and meaningful image interpolation.

==> sections/background.tex <==
\subsection{Preliminary}
\label{subsec:background}
\lc{\st{move up the related work. And move the background as preliminary to section 3;} Do we need all those equations? And, if we don't refer back those equations, we shall simply take out the number}

\textbf{Reverse process:} The optimization objective of diffusion models \cite{sohl2015deep} is derived by variational inference. Given the observed data $\boldsymbol{x}_0$, the diffusion model is a probabilistic model which specifies the joint distribution $p_\theta(\boldsymbol{x}_{0: T})$, where $\boldsymbol{x}_1, ..., \boldsymbol{x}_T$ are latent variables that have the same dimensions as $\boldsymbol{x}_0$ and $\theta$ is the learnable model parameters. $p_\theta(\boldsymbol{x}_{0: T})$ is defined as a Markov chain that samples from $\boldsymbol{x}_T$ to $\boldsymbol{x}_0$:
\begin{equation}
    p_\theta\left(\boldsymbol{x}_{0: T}\right):=p_{\theta}\left(\boldsymbol{x}_T\right) \prod_{t=1}^T p_\theta\left(\boldsymbol{x}_{t-1} \mid \boldsymbol{x}_t\right).
\end{equation}
Denoising diffusion probabilistic model (DDPM) \cite{ddpm:ho2020denoising} assumes that $p_{\theta}\left(\boldsymbol{x}_T\right)=\mathcal{N}\left(\boldsymbol{x}_T ; \mathbf{0}, \boldsymbol{I}\right)$ and
\begin{equation}
  p_\theta\left(\boldsymbol{x}_{t-1} \mid \boldsymbol{x}_t\right)=\mathcal{N}\left(\boldsymbol{x}_{t-1} ; \boldsymbol{\mu}_\theta\left(\boldsymbol{x}_t, t\right), \sigma_t^2 \boldsymbol{I}\right), 
  \label{eq:pt1t}
\end{equation}
where $\sigma_t \in \mathbb{R}_{\geq 0}$. In diffusion model, the Markov chain $p_\theta(\boldsymbol{x}_{0: T})$ is called the \textit{reverse process}. It gradually denoises a noise $\boldsymbol{x}_T \sim \mathcal{N}\left(\boldsymbol{x}_T ; \mathbf{0}, \boldsymbol{I}\right)$. 

\textbf{Forward process: }For deriving a lower bound on the log likelihood of the observed data, diffusion models introduce the approximate posterior $q\left(\boldsymbol{x}_{1: T} \mid \boldsymbol{x}_0\right)$ which is a Markov chain that samples from $\boldsymbol{x}_1$ to $\boldsymbol{x}_T$:
\begin{equation}
    q\left(\boldsymbol{x}_{1: T} \mid\boldsymbol{x}_0\right):=\prod_{t=1}^T q\left(\boldsymbol{x}_t \mid \boldsymbol{x}_{t-1}\right).
\end{equation}
Then the log data likelihood can be decomposed as $\mathbb{E}\left[\log p_\theta\left(\boldsymbol{x}_0\right)\right] = \mathbb{E}_q\left[\log \frac{p_\theta\left(\boldsymbol{x}_{0: T}\right)}{q\left(\boldsymbol{x}_{1: T} \mid \boldsymbol{x}_0\right)}\right] + D_{\mathrm{KL}}\left(q\left(\boldsymbol{x}_{1:T} \mid \boldsymbol{x}_0\right) \| p_\theta\left(\boldsymbol{x}_{1:T} \mid \boldsymbol{x}_0 \right)\right)$. Thus, we have the lower bound $\mathbb{E}\left[\log p_\theta\left(\boldsymbol{x}_0\right)\right] \geq \mathbb{E}_q\left[\log \frac{p_\theta\left(\boldsymbol{x}_{0: T}\right)}{q\left(\boldsymbol{x}_{1: T} \mid \boldsymbol{x}_0\right)}\right]$. When training the diffusion model, for maximizing $\mathbb{E}\left[\log p_\theta\left(\boldsymbol{x}_0\right)\right]$, the parameters $\theta$ are learned to minimize the negative evidence lower bound:
\begin{equation}
    \mathop{\arg\min}_{\theta} \mathbb{E}_{q}\left[\log q\left(\boldsymbol{x}_{1: T} \mid \boldsymbol{x}_0\right)-\log p_\theta\left(\boldsymbol{x}_{0: T}\right)\right].
    \label{eq:loss}
\end{equation}
The Markov chain  $q\left(\boldsymbol{x}_{1: T} \mid \boldsymbol{x}_0\right)$ is called the \textit{forward process}, which progressively turns the data $x_0$ into noise. The conditional distribution in each forward step is defined as:
\begin{equation}
    q\left(\boldsymbol{x}_t \mid \boldsymbol{x}_{t-1}\right):=\mathcal{N}\left(\boldsymbol{x}_t; \sqrt{\frac{\alpha_t}{\alpha_{t-1}}} x_{t-1},\left(1-\frac{\alpha_t}{\alpha_{t-1}}\right) \boldsymbol{I}\right),
    \label{eq:qtt1}
\end{equation}
where $\alpha_t \in (0,1]$ and $\alpha_{1}, ..., \alpha_T$ is a decreasing sequence, which ensures that the values on the diagonal of the covariance matrix are positive. By reparameterization using the definition in Eq.~(\ref{eq:qtt1}), an important property of the forward process is that:
\begin{equation}
    q\left(\boldsymbol{x}_t \mid \boldsymbol{x}_0\right) = \mathcal{N}\left(\boldsymbol{x}_t ; \sqrt{\alpha_t} \boldsymbol{x}_0,\left(1-\alpha_t\right) \boldsymbol{I}\right).
\end{equation}

\textbf{Training and sampling: }According to the definition of the reverse process $p$ and the forward process $q$, $\alpha_t$ and $\sigma_t$ for all $t$ are not learnable parameters. Thus, DDPM simplifies Eq.~(\ref{eq:loss}) as:
\begin{equation}
    \mathop{\arg\min}_{\theta} \sum_t \mathbb{E}_q [D_{\mathrm{KL}}\left(q\left(\boldsymbol{}{x}_{t-1} \mid \boldsymbol{x}_t, \boldsymbol{x}_0\right) \| p_\theta\left(\boldsymbol{x}_{t-1} \mid \boldsymbol{x}_t\right)\right)].
    \label{eq:loss_sim}
\end{equation}
We further choose the form of $\boldsymbol{\mu}_\theta\left(\boldsymbol{x}_t, t\right)$ to be:
\begin{equation}
    \boldsymbol{\mu}_\theta\left(\boldsymbol{x}_t, t\right) = \frac{1}{\sqrt{\frac{\alpha_t}{\alpha_{t-1}}}}\left(\boldsymbol{x}_t-\frac{1-\frac{\alpha_t}{\alpha_{t-1}}}{\sqrt{1-\alpha}_t} \boldsymbol{\epsilon}_\theta\left(\boldsymbol{x}_t, t\right)\right),
    \label{eq:pmean}
\end{equation}
where $\boldsymbol{\epsilon}_\theta$ is a function with trainable parameters $\theta$. According to the above definitions on the forward process and the reverse process and applying the parameterization shown in Eq.~(\ref{eq:pmean}), Eq.~(\ref{eq:loss_sim}) can be simplified as $\mathop{\arg \min}_{\theta} L(\theta)$, where:
\begin{equation}
\footnotesize
    L(\theta):= \sum_{t=1}^{T} \mathbb{E}_{\mathbf{x}_0, \boldsymbol{\epsilon}_t}\left[\gamma_t\left\|\boldsymbol{\epsilon}_t-\boldsymbol{\epsilon}_\theta\left(\sqrt{\alpha_t} \mathbf{x}_0+\sqrt{1-\alpha}_t \boldsymbol{\epsilon}_t, t\right)\right\|^2\right],
\end{equation}
where $\gamma_t = \frac{(\alpha_{t-1}-\alpha_t)^2}{2 \sigma_t^2 \alpha_t \alpha_{t-1}(1-\alpha_t)}$ and $\boldsymbol{\epsilon}_t \sim \mathcal{N}(\mathbf{0}, \boldsymbol{I})$. \cite{ddpm:ho2020denoising} simplifies further the training objective $L$ by setting $\gamma_t = 1$ instead of depending on $\alpha_{1:T}$.

The number of sampling steps $T$ decides the generalization capability and the sampling cost of diffusion models. A big $T$ leads to a reverse process with high generalization capability and better capture the pattern of $x_0$. However, it also increases the sampling time and makes the sampling from DDPMs significantly slower than other generative models, e.g, GANs. Such inefficiency promotes our design of \alg for distillation into smaller sampling steps.










==> sections/introduction.tex <==
\label{sec:introduction}

Generative models, such as Generative Adversarial Networks (GANs) and Variational Autoencoders (VAEs), are 
successfully applied to synthesize data for a wide spectrum of applications, including audio synthesis~\cite{audio:conf/icml/MarafiotiPHM19}, text-to-image~\cite{text2image:conf/icml/ChangZBML00MFRL23,text2image:conf/icml/SauerKL0A23} and synthetic image generation~\cite{generation:conf/icml/0005FBNLVSB23}. 
Recently, diffusion models~\cite{song2020score, ho2022cascaded, ddpm:ho2020denoising} emerge and generate images of exceptional high quality, without the necessity of conducting adversarial training.
% outperforming state-of-the-art GANs (e.g., BigGAN-deep~\cite{biggandeep:conf/iclr/BrockDS19}) and VAEs (e.g., VQ-VAE-2~\cite{vqvae2:conf/nips/RazaviOV19}) \lc{Make sure they are really the best and VAE is really not considered as the state of the art}.
% Diffusion models learn to synthesize data by gradually noising the training data and then reconstruct the data by reversing the process.
The diffusion models constitute a Markov chain of forward steps of slowly adding random noise to data, followed by a reverse process in which the data is gradually reconstructed from the noise. The underlying networks typically use the UNet architecture to better connect the forward steps to the corresponding denoise steps. However, an important hindrance is that such models require large numbers of sampling steps, e.g., 1000 steps in DDPM~\cite{ddpm:ho2020denoising}, which {leads to high sampling/inference\footnote{We interchange the use of sampling and inference time. } times limiting}  their practical applications on real time computation. %\rb{Why? High compute costs? be more explicit also to better introduce the next paragraph, e.g. what does smapling time refer to?}

%\rb{You need to add a brief description of what each of these techniques actually does}
To reduce the sampling time of diffusion models and maintain the quality of image synthesis, there are several directions explored by the prior art. One approach is to compress the UNet ~\cite{li2023snapfusion, zhao2023mobilediffusion} and combine the acceleration technologies of GPU. The other approach is to reduce the sampling steps, as inference time of diffusion models linearly correlates to the number of sampling steps. ~\citet{ddim:conf/iclr/SongME21} skips intermediate steps under generalizing the original Markovian process via a class of non-Markovian diffusion steps. The above approaches do not change the original training procedure. On the other hand, progressive distillation~\cite{progress:salimans2022progressive,meng2023distillation} introduces a teacher-student framework to reduce a trained teacher diffusion model of $T$ steps into a student diffusion of $T'$ steps, where $T' \ll T$, via multiple binary foldings by retraining. For instance, distilling a 1024-step diffusion model into a 128-step model needs to first train a 512-step intermediate model, then a 256-step, to finally arrive to the 128-step model. The distillation objective is to minimize the output differences between teacher and student model. While progressive distillation better maintains the synthesis quality than step-skipping, it incurs high distillation time and is limited by the restrictions on $T$ and $T'$ due to the binary folding.

% To reduce the sampling time while keeping high sampling quality, one can optimize the UNet~\cite{li2023snapfusion, zhao2023mobilediffusion}, for fast sampling, e.g., with reparameterization~\cite{}, which %\stef{does the which refer to reparameterization or fast sampling?} \gill{reparameterization} 
% can also be plugged into other acceleration techniques%\rb{we did not mention yet our aims}. 
% Also, skipping intermediate inference steps is applicable when generalizing the original Markovian process via a class of non-Markovian diffusion steps~\cite{ddim:conf/iclr/SongME21} %\stef{is it really generalizing if we replace Markovian with non-Markovian? what are we generalizing to? from markovian to general stochastic process?}, 
% while %\stef{not sure if while is what you want here} suffering from plummeted synthetic data quality with 
% excessive skipped sampling steps. Additionally, progressive distillation~\cite{progress:salimans2022progressive,meng2023distillation} enables progressive binary folding of the original model into a lower number of  steps. For instance, distilling a 1024-step diffusion models into a 128-step model needs to first get a 512-step model, then 256-step, and finally arrives to 128-step model.  However, the binary folding has restricted functionality \stef{in what sense? does it only maintain a subset of the functionality?} of the original deterministic diffusion sampler with binary exponential steps.

In this paper, our objective is to design an effective distillation method which achieves high quality in (any) small sampling step and concurrently incurs low distillation time.
We propose, \alg, a single-fold distillation framework, reducing a $T$-step teacher diffusion model into a $T'$-step student diffusion model in a single-fold optimization. Thanks to its single-fold nature, \alg offers the great flexibility on distilling teacher model of any arbitrary steps. To such an end, we first define a new student model, which can extract knowledge of the teacher diffusion model, by an arbitrary sub-sequence. Our definition on forward process solves the challenge of aligning the variables of teacher and student models, enabling flexible single-fold distillation. Secondly, when training the denoise process of the student model, we minimize not only the output difference but also the hidden variables difference of the sampling steps between teacher and student model to better preserve the image synthesis quality.

To demonstrate the effectiveness, we evaluate \alg against sampling-skip~\cite{ddim:conf/iclr/SongME21} and progressive distillation~\cite{progress:salimans2022progressive} on CIFAR-10, CelebA, LSUN-Church, and LSUN- Bedroom~datasets. We compare their synthesis quality in terms of Fr\'{e}chet Inception Distance (FID)~\cite{fid:conf/nips/HeuselRUNH17} of distilling a 1024-step diffusion model into 128-step and 16-step models. \alg achieves the lowest FID as well as the best perceptual quality, also with flexibility on the numerical relation between the teacher and the student, i.e., works for both 1024 to 128 or 100 steps. Further, the distillation effectiveness is validated on semantic input-output consistency and image interpolation.

We summarize the contributions of this paper as follows: %\dick{I prefer a uniform style with all contributions starting with ``We [verb] ...". Also, you may add to each contribution ``(Section X)" with its place in the paper.}
% \stef{switching between present and past tense, please be consistent}

%$$ we define the curtailed student forward process by extracting knowledge from an arbitrary sub-sequence of the teacher DDPM-like diffusion models. Then, the underlying probability distributions on the hidden variables of the sampling steps are imitated accordingly in the reverse process. The knowledge of the teacher diffusion model is hence  transferred to the lightweight student model for faster inference. For validating the effectiveness of the proposed method, we conduct experiments on CIFAR-10~\cite{cifar:krizhevsky2009learning}, CelebA~\cite{celeba:liu2015faceattributes}, LSUN-Church, and LSUN- Bedroom~\cite{lsun:yu15lsun} datasets. The results demonstrate that \gill{add} ...
%We summarize the contributions of this paper as follows: \dick{I prefer a uniform style with all contributions starting with ``We [verb] ...". Also, you may add to each contribution ``(Section X)" with its place in the paper.}
% \stef{switching between present and past tense, please be consistent}
\begin{itemize}
    \item %Instead of several foldings, 
    We propose a novel single-fold distillation algorithm, \alg, which can agilely  compress teacher diffusion into a student diffusion model of any step in one fold.
    \item We define a new forward process for student diffusion, which aligns and approximates student and teacher Markovian variables, enabling flexible single-fold distillation.
    \item We design effective training for student diffusion by minimizing the difference of output and hidden variables with respect to the teacher diffusion.  
    \item We experimentally demonstrate superiority of \alg in achieving high-quality sampling data by as little as approximately 1\% number of steps.
    % using significantly lower distillation computation. %\stef{this sentence sounds like we achieve better FID and perceptual quality but up to now, the introduction mainly sells that we are faster; did we not also evaluate computation time or something like that? }\gill{our selling point is faster than the teacher, higher FID and perceptual quality than other acceleration baselines}. 
\end{itemize}


% Besides, the training of diffusion process mitigates instability in practice, by designed in continuous latent spaces, compared with GANs \cite{ho2020denoising}in discrete pixel spaces, requiring very specific choices in optimization and architectures to stabilize training. 



% However, when generating a synthetic image, diffusion model requires to produce lots of intermediate hidden variables that is computational intensive. The complex architecture of diffusion models increases the sampling time. This weakness prevents the application of diffusion models in some scenarios with limited computing resources, e.g., edge devices.

% To address the problem of slow sampling time on diffusion models. Recent prior arts \cite{salimans2022progressive, meng2023distillation} utilize model distillation to reduce the number of sampling steps. \lc{Need to introduce how teacher-student work for distillation}Given a trained big teacher model, model distillation is applied to extract the knowledge from the teacher and yield a smaller student model with few sampling steps and smaller model size while ensuring similar synthetic image quality between the teacher and the student. The authors proposed a method named progressive distillation to always half the number of sampling steps in each round of distillation, e.g., distilling a trained N-step DDIM model \cite{ho2020denoising} into a new model with $N/2$ steps. The distillation method is letting the student mimic the intermediate outputs of the teacher on half of the teacher's steps. \gill{what is the drawback} \lc{The point is the progressive halving algorithm. We need to clearly stress limitations of prior art: only align the output and progressive halfving} 

% In this paper, we argue that merely mimicking the intermediate outputs of the teacher diffusion model is not enough to fully extract the knowledge from the teacher. Since there are multiple underlying probability distributions on the hidden variables of the sampling steps, a distillation algorithm can actually also approximates the distributions of the trained teacher so as to thoroughly learn its knowledge. We propose an algorithm based on this idea named XXX.




% \clearpage

==> sections/methodology.tex <==
\begin{figure*}[!ht]
	\centering
	{       \includegraphics[width=0.95\textwidth]{icml2024/imgs/diffusion_distilation_drawio.pdf} }
	\caption{Single-folding diffusion model distillation (\alg). The student accelerates the inference by a small $T^{\prime}$ (e.g., $T^{\prime} = 16$, 3 in the figure) sampling steps instead of a large $T$ (e.g., $T=1024$, 9 in the figure) of the teacher while keeping sampling quality. The distribution of $\boldsymbol{x}^{\prime}_t$ approximates the distribution of $\boldsymbol{x}_{ct}$, where $c = T/T^{\prime}$ and $c \in \mathbb{Z}$. To align the teacher and student Markov chains, we propose to match the intermediate hidden variables to make $q^{\prime}(\boldsymbol{x}^{\prime}_t = \boldsymbol{x}_{ct} \mid \boldsymbol{x}^{\prime}_0 = \boldsymbol{x}_0)$ equal to $q(\boldsymbol{x}_{ct}|\boldsymbol{x}_0)$. Note that here $T^{\prime}$ is divisible by $T$ but we will release this constraints in Sec.~\ref{subsec:flexible}.  }
        \label{fig:graph_model}
\end{figure*}
\label{sec:methodology}
\lc{\st{When glancing this section, I can not quickly find the novelties of the proposed algorithm, matching the hiddent state. As of now, the description is very much bottom up. The other things to stress are the difference of derivation of student model from the original derivation of "teacher model" and their training procedure. For the original diffusion training, we can train any random t but not here. }}
% In practical deployment scenarios, the inference latency and the required computation amount are important  \gill{Do we need this sentence in the beginning of methodology?}.
% In order to reduce the number of sampling steps, we propose a knowledge distillation algorithm. Given a trained diffusion model that has a large $T$ (e.g., $T = 1024$) steps, the algorithm extracts the knowledge from it into a faster diffusion model that has $T^{\prime}$ sampling steps while keep the same quality, where $T^{\prime} \ll T$, e.g., $T^{\prime} = 4$. In this paper we call the trained diffusion model as the \textit{teacher} model and the faster one as the \textit{student} model. 

% \subsection{Challenge and design of diffusion model distillation}
\subsection{Single-fold DDM \alg}

First, we define how to distill the student model according to the \textbf{trained} parameters and settings of the teacher, instead of training from scratch from the observed data $\mathcal{D} = \{x_0\}$.
Following Sec.~\ref{subsec:background}, the variable sequence observed from the teacher is denoted as $\boldsymbol{x}_0,...,\boldsymbol{x}_T$, where $\boldsymbol{x}_T$ is the input of the reverse process, $\boldsymbol{x}_0$ is the output and $\boldsymbol{x}_1,...,\boldsymbol{x}_{T-1}$ are the corresponding latent values on the Markov chain.
Accordingly, the variables of the student are $\boldsymbol{x}^{\prime}_0,...,\boldsymbol{x}^{\prime}_{T^{\prime}}$, where $T^{\prime} \ll T$. Our goal is to distill the knowledge of the teacher model by mimicking hidden variables ($\boldsymbol{x}_0,...,\boldsymbol{x}_T$) as well as the final output by compressed sub-sequence ($\boldsymbol{x}^{\prime}_0,...,\boldsymbol{x}^{\prime}_{T^{\prime}}$).

As shown in Fig.~\ref{fig:graph_model}, in order to mimic the teacher distributions by discrete sub-sequence, one challenge comes from mapping in continuous\gill{unsure which word to use} Markovian steps. For example, given an index $ct$, according to Sec.~\ref{subsec:background}, the distributions we can explicitly obtain from the teacher is $q\left(\boldsymbol{x}_{ct} \mid \boldsymbol{x}_{ct-1}\right)$ (see Eq.~\ref{eq:qtt1}) and $p_\theta\left(\boldsymbol{x}_{ct-1} \mid \boldsymbol{x}_{ct}\right)$ (see Eq.~\ref{eq:pt1t} and Eq.~\ref{eq:pmean}).
However, mapping $\boldsymbol{x}^{\prime}_t$ with $\boldsymbol{x}_{ct}$ from the student to the teacher does not holds for the next step, i.e., $\boldsymbol{x}^{\prime}_{t-1}$ does not correspond to $\boldsymbol{x}_{ct-1}$, which is supposed to map $\boldsymbol{x}_{c(t-1)}$. Thus, when distilling the DDPM-like Markov chains, it is not reasonable to simply and straightforwardly simulate $q^{\prime}(\boldsymbol{x}^{\prime}_t|\boldsymbol{x}^{\prime}_{t-1})$ as $q(\boldsymbol{x}_{ct}|\boldsymbol{x}_{ct-1})$ while estimating $p^{\prime}_{\Theta}(\boldsymbol{x}^{\prime}_t|\boldsymbol{x}^{\prime}_{t-1})$ as $p_{\theta}(\boldsymbol{x}_{ct}|\boldsymbol{x}_{ct-1})$, where the notations $q^{\prime}$ and $p^{\prime}_{\Theta}$ are used to represent the forward process and reverse process of the student model respectively.


% Instead of training the student model from scratch just relying on the observed data $\mathcal{D} = \{x_0\}$, we define and train the student model according to the trained parameters and settings of the teacher model. The variable sequence observed from the trained teacher is denoted as $\boldsymbol{x}_0,...,\boldsymbol{x}_T$, where $\boldsymbol{x}_T$ is the input of the generative process, $\boldsymbol{x}_0$ is the output and $\boldsymbol{x}_1,...,\boldsymbol{x}_{T-1}$ are the corresponding latent values on the Markov chain. In order to distinguish the student from the teacher\gill{do not find this sentence necessary}, the variables of the student are represented by $\boldsymbol{x}^{\prime}_0,...,\boldsymbol{x}^{\prime}_{T^{\prime}}$. As shown in Fig.~\ref{fig:graph_model}, $\boldsymbol{x}^{\prime}_t$ corresponds to $\boldsymbol{x}_{ct}$, where $c = T/T^{\prime}$. When training the student, besides letting $\boldsymbol{x}^{\prime}_t$ mimic $\boldsymbol{x}_{ct}$ so as to copy the model outputs (including the intermidiate outputs) of the teacher, we also want to extract the knowledge from the teacher's distributions. However, given an index $ct$, the distributions we can directly obtain from the teacher is $q\left(\boldsymbol{x}_{ct} \mid \boldsymbol{x}_{ct-1}\right)$ (see Eq.~\ref{eq:qtt1}) and $p_\theta\left(\boldsymbol{x}_{ct-1} \mid \boldsymbol{x}_{ct}\right)$ ( see Eq.~\ref{eq:pt1t} and Eq.~\ref{eq:pmean}). Although $\boldsymbol{x}_{ct}$ can be mapped to $\boldsymbol{x}^{\prime}_t$, but $\boldsymbol{x}_{ct-1}$ does not correspond to $\boldsymbol{x}^{\prime}_{t-1}$. Thus, when distilling the Markov chains, it is not reasonable to simply and straightforwardly simulate $q^{\prime}(\boldsymbol{x}^{\prime}_t|\boldsymbol{x}^{\prime}_{t-1})$ as $q(\boldsymbol{x}_{ct}|\boldsymbol{x}_{ct-1})$ while estimate $p^{\prime}_{\Theta}(\boldsymbol{x}^{\prime}_t|\boldsymbol{x}^{\prime}_{t-1})$ as $p_{\theta}(\boldsymbol{x}_{ct}|\boldsymbol{x}_{ct-1})$, where the notations $q^{\prime}$ and $p^{\prime}_{\Theta}$ are respectively used to represent the forward process and reverse process of the student model.

To overcome the above challenge, our idea for defining the novel student model as follows. Note that the key definition for diffusion models is the forward process $q^{\prime}\left(\boldsymbol{x}^{\prime}_{1: T^{\prime}} \mid \boldsymbol{x}^{\prime}_0\right)$, as it determines the variational inference and training of the model. Therefore, for better copying the knowledge from the teacher, we design $q^{\prime}\left(\boldsymbol{x}^{\prime}_{1: T^{\prime}} \mid \boldsymbol{x}^{\prime}_0\right)$ by extracting the teacher's forward process $q\left(\boldsymbol{x}_{1: T} \mid \boldsymbol{x}_0\right)$. Specifically, while extracting the Markov chain $q$, to ensure correspondence between the latent variables in the two diffusion models, given any $t \in [1, T^{\prime}]$, the proposed distillation algorithm \textbf{aims} to make $q^{\prime}(\boldsymbol{x}^{\prime}_t = \boldsymbol{x}_{ct} \mid \boldsymbol{x}^{\prime}_0 = \boldsymbol{x}_0)$ equal to $q(\boldsymbol{x}_{ct}|\boldsymbol{x}_0)$. After fixing $q^{\prime}$ by such approximation in the forward process, the reverse process of the student is constructed accordingly. In the following, we show in detail how to define a corresponding student model that extracts a given DDPM teacher model defined in Sec~\ref{subsec:background}.
% The key definition for diffusion models is the forward process $q^{\prime}\left(\boldsymbol{x}^{\prime}_{1: T^{\prime}} \mid \boldsymbol{x}^{\prime}_0\right)$ definition is crucial, because it decides the variational inference and training of the model. In the proposed distillation algorithm, for better copying the knowledge from the teacher, we design $q^{\prime}\left(\boldsymbol{x}^{\prime}_{1: T^{\prime}} \mid \boldsymbol{x}^{\prime}_0\right)$ by extracting the teacher's forward process $q\left(\boldsymbol{x}_{1: T} \mid \boldsymbol{x}_0\right)$. When extracting the Markov chain $q$, to ensure correspondence between the latent variables in the two diffusion models, given any $t \in [1, T^{\prime}]$, the proposed distillation algorithm aims to make $q^{\prime}(\boldsymbol{x}^{\prime}_t = \boldsymbol{x}_{ct} \mid \boldsymbol{x}^{\prime}_0 = \boldsymbol{x}_0)$ equal $q(\boldsymbol{x}_{ct}|\boldsymbol{x}_0)$. After fixing $q^{\prime}$ by the extraction, the reverse process of the student is constructed accordingly. In the following, given a DDPM teacher model defined as shown in the backround section, we show how to choose a corresponding student model and extract the knowledge from the teacher.

\subsection{The forward process of the student model}
\ch{\st{highlight why we design the forward process of the student in this way - we want to make sure a property that $q^{\prime}(\boldsymbol{x}^{\prime}_t = \boldsymbol{x}_{ct} \mid \boldsymbol{x}^{\prime}_0 = \boldsymbol{x}_0)$ equals $q(\boldsymbol{x}_{ct}|\boldsymbol{x}_0)$}}

\gill{check}


To distill the DDPM teacher, we also assume that the student model has a Markovian forward process. \gill{single-folding} Thus  $q^{\prime}\left(\boldsymbol{x}^{\prime}_{1: T^{\prime}} \mid \boldsymbol{x}^{\prime}_0\right)$ is a Markov chain that can be factorized as $$q^{\prime}\left(\boldsymbol{x}^{\prime}_{1: T^{\prime}} \mid \boldsymbol{x}^{\prime}_0\right):=\prod_{t=1}^{T^{\prime}} q^{\prime}\left(\boldsymbol{x}^{\prime}_t \mid \boldsymbol{x}^{\prime}_{t-1}\right).$$ 
As shown in Eq.~(\ref{eq:qtt1}), the forward process of the teacher is defined by a decreasing sequence $\alpha_{1}, ..., \alpha_T$. As for the student, different from the Gaussian distribution shown in Eq.~(\ref{eq:qtt1}), we set the student's forward process as the following distribution:
\begin{equation}
\footnotesize
q^{\prime}\left(\boldsymbol{x}^{\prime}_t \mid \boldsymbol{x}^{\prime}_{t-1}\right):=\mathcal{N}\left(\boldsymbol{x}^{\prime}_t; \sqrt{\frac{\alpha_{ct}}{\alpha_{ct-c}}} x^{\prime}_{t-1},\left(1-\frac{\alpha_{ct}}{\alpha_{ct-c}}\right) \boldsymbol{I}\right),
    \label{eq:qtt1s}
\end{equation}
for all $t \in [1,T^{\prime}]$ based on the elements of the sequence. Then, according to this forward process definition of the student, we have the property:
\begin{equation}
q^{\prime}(\boldsymbol{x}^{\prime}_t \mid \boldsymbol{x}^{\prime}_0) =  \mathcal{N}\left(\boldsymbol{x}^{\prime}_t ; \sqrt{\alpha_{ct}} \boldsymbol{x}^{\prime}_0,\left(1-\alpha_{ct}\right) \boldsymbol{I}\right).
\label{eq:qxtx0}
\end{equation}
It \textbf{ensures} that $q^{\prime}(\boldsymbol{x}^{\prime}_t = \boldsymbol{x}_{ct} \mid \boldsymbol{x}^{\prime}_0 = \boldsymbol{x}_0) = q(\boldsymbol{x}_{ct}|\boldsymbol{x}_0)$, where $\boldsymbol{x}^{\prime}_t$ corresponds to $\boldsymbol{x}_{ct}$ (see Lemma 1 of Appendix~\ref{app:proofs}). Thus, the student's Markov chain $q^{\prime}\left(\boldsymbol{x}^{\prime}_{1: T^{\prime}} \mid \boldsymbol{x}^{\prime}_0\right)$ can be regarded as a simplified copy of the teacher's forward process $q\left(\boldsymbol{x}_{1: T} \mid \boldsymbol{x}_0\right)$.

Before introducing the reverse process, we derive some important forward process posteriors. Applying Bayes' rule:
\begin{equation*}
    q^{\prime}\left(\boldsymbol{x}^{\prime}_{t-1} \mid \boldsymbol{x}^{\prime}_t, \boldsymbol{x}^{\prime}_0\right)=q^{\prime}\left(\boldsymbol{x}^{\prime}_t \mid \boldsymbol{x}^{\prime}_{t-1}, \boldsymbol{x}^{\prime}_0\right) \frac{q^{\prime}\left(\boldsymbol{x}^{\prime}_{t-1} \mid \boldsymbol{x}^{\prime}_0\right)}{q^{\prime}\left(\boldsymbol{x}^{\prime}_t \mid \boldsymbol{x}^{\prime}_0\right)},
\end{equation*}
and the Markov chain property that $q^{\prime}\left(\boldsymbol{x}^{\prime}_t \mid \boldsymbol{x}^{\prime}_{t-1}, \boldsymbol{x}^{\prime}_0\right) = q^{\prime}\left(\boldsymbol{x}^{\prime}_t \mid \boldsymbol{x}^{\prime}_{t-1}\right)$, we have the following posteriors
\begin{equation}
\footnotesize
\begin{aligned}
    &q^{\prime}\left(\boldsymbol{x}^{\prime}_{t-1} \mid \boldsymbol{x}^{\prime}_t, \boldsymbol{x}^{\prime}_0\right) =  \\ 
    &\mathcal{N}\left(\boldsymbol{x}^{\prime}_{t-1} ; \frac{(1-\alpha_{ct-c})\sqrt{\alpha_{ct}}}{(1-\alpha_{ct})\sqrt{\alpha_{ct-c}}}\boldsymbol{x}^{\prime}_t + \frac{\alpha_{ct-c}-\alpha_{ct}}{(1-\alpha_{ct})\sqrt{\alpha_{ct-c}}}\boldsymbol{x}^{\prime}_0, \sigma^{\prime}_t \boldsymbol{I}\right),
\end{aligned}
\label{eq:qposter}
\end{equation}
where $\sigma^{\prime}_t = \frac{(1-\alpha_{ct-c})(\alpha_{ct-c}-\alpha_{ct})}{(1-\alpha_{ct})\alpha_{ct-c}}$ (see Appendix \gill{idx} for the derivation). 


\subsection{The reverse process of the student model}

\gill{check}

In the following, we define the reverse process of the student model according to the teacher model. Similarly, it is also a Markov chain represented as  $p^{\prime}_\Theta(\boldsymbol{x}^{\prime}_{0: T^{\prime}}) := p^{\prime}_{\Theta}\left(\boldsymbol{x}^{\prime}_T\right) \prod_{t=1}^{T^{\prime}} p^{\prime}_\Theta\left(\boldsymbol{x}^{\prime}_{t-1} \mid \boldsymbol{x}^{\prime}_t\right),$ where $p^{\prime}_{\Theta}\left(\boldsymbol{x}^{\prime}_T\right) = \mathcal{N}\left(\boldsymbol{x}^{\prime}_T ; \mathbf{0}, \boldsymbol{I}\right)$ and $\Theta$ represents the learnable parameters of the student. 

Specifically, we then decide the form of $p^{\prime}_\Theta\left(\boldsymbol{x}^{\prime}_{t-1} \mid \boldsymbol{x}^{\prime}_t\right)$.
Using Eq.~(\ref{eq:qxtx0}), we can reparameterize $\boldsymbol{x}^{\prime}_t$ as a linear combination of $\boldsymbol{x}^{\prime}_0$ and $\epsilon_t \sim \mathcal{N}(\mathbf{0}, \boldsymbol{I})$ that $\boldsymbol{x}^{\prime}_t=\sqrt{\alpha_{ct}} \boldsymbol{x}^{\prime}_0+\sqrt{1-\alpha_{ct}} \epsilon_t$. Let the model $\epsilon^{\prime}_{\Theta}(\boldsymbol{x}^{\prime}_t, t)$ predict $\epsilon_t$, we have a prediction of $\boldsymbol{x}^{\prime}_0$ given $\boldsymbol{x}^{\prime}_t$:

\begin{equation}
f_\Theta^{(t)}\left(\boldsymbol{x}^{\prime}_t\right):=\left(\boldsymbol{x}^{\prime}_t-\sqrt{1-\alpha_{ct}} \cdot \epsilon^{\prime}_\Theta\left(\boldsymbol{x}^{\prime}_t,t\right)\right) / \sqrt{\alpha_{ct}}
\end{equation}

According to Eq.~(\ref{eq:loss_sim}), we know that in the student diffusion model, $p^{\prime}_\Theta\left(\boldsymbol{x}^{\prime}_{t-1} \mid \boldsymbol{x}^{\prime}_t\right)$ is a distribution that predicts $q^{\prime}(\boldsymbol{x}^{\prime}_{t-1} \mid \boldsymbol{x}^{\prime}_t, \boldsymbol{x}^{\prime}_0)$. Thus, we define that for all $t \in [1, T^{\prime}]$,
\begin{equation}
    p^{\prime}_\Theta\left(\boldsymbol{x}^{\prime}_{t-1} \mid \boldsymbol{x}^{\prime}_t\right) = q^{\prime}(\boldsymbol{x}^{\prime}_{t-1} \mid \boldsymbol{x}^{\prime}_t, f_\Theta^{(t)}\left(\boldsymbol{x}^{\prime}_t\right)).
    \label{eq:pdef}
\end{equation}
Then, based on Eq.~(\ref{eq:qposter}) and Eq.~(\ref{eq:pdef}), by replacing $\boldsymbol{x}^{\prime}_0$ as the predictor $f_\Theta^{(t)}\left(\boldsymbol{x}^{\prime}_t\right)$, we have: 
\begin{equation}
     p^{\prime}_\Theta\left(\boldsymbol{x}^{\prime}_{t-1} \mid \boldsymbol{x}^{\prime}_t\right) =  \mathcal{N}\left(\boldsymbol{x}^{\prime}_{t-1} ; \boldsymbol{\mu}^{\prime}_\Theta\left(\boldsymbol{x}^{\prime}_t, t\right), \sigma^{\prime}_t \boldsymbol{I}\right),
     \label{eq:pt1t}
\end{equation}
where the mean:
\begin{equation}
\footnotesize
\boldsymbol{\mu}^{\prime}_\Theta\left(\boldsymbol{x}^{\prime}_t, t\right) = \frac{(1-\alpha_{ct-c})\sqrt{\alpha_{ct}}}{(1-\alpha_{ct})\sqrt{\alpha_{ct-c}}}\boldsymbol{x}^{\prime}_t + \frac{\alpha_{ct-c}-\alpha_{ct}}{(1-\alpha_{ct})\sqrt{\alpha_{ct-c}}}f_\Theta^{(t)}\left(\boldsymbol{x}^{\prime}_t\right).
\end{equation}

\gill{maybe add one sentence of summarizing reverse process or property}

\subsection{Training and sampling}

\gill{check}

After the definition of the forward and reverse process of the student model, here we design the deployment for training and sampling.
In our distillation algorithm, we want to train a student by extracting the knowledge from a trained teacher. Thus, instead of minimizing the Kullback-Leibler divergence between Eq.~(\ref{eq:qposter}) and Eq.~(\ref{eq:pt1t}) and come up with a training loss which is only based on data $\{x_0\}$, we propose to train the student based on the teacher's outputs in all the steps $\boldsymbol{x}_0,...,\boldsymbol{x}_T$. \gill{sub-sequence steps or all steps}

\textbf{Training:} The basic idea is that, given any index $t \in [0,T^{\prime}]$, we let the student's variable $\boldsymbol{x}^{\prime}_t$ mimic the teacher's variable $\boldsymbol{x}_{ct}$. First, we let $\boldsymbol{x}^{\prime}_{T^{\prime}} = \boldsymbol{x}_{T}$. Then the student gradually sample $\boldsymbol{x}^{\prime}_{T^{\prime}-1}$ to $\boldsymbol{x}^{\prime}_0$ while for each $\boldsymbol{x}^{\prime}_t$ the student is optimized by minimizing the distance $\|\boldsymbol{x}^{\prime}_t-\boldsymbol{x}_{ct}\|^{2}$. Algorithm~\ref{aaaaa} illustrate the training procedure of the student.

\textbf{Sampling:} Since the reverse process of the student is defined by Eq.~(\ref{eq:pt1t}), given $\boldsymbol{x}^{\prime}_{T^{\prime}}$, we can progressively sample all the variables from $\boldsymbol{x}^{\prime}_{T^{\prime}-1}$ to $\boldsymbol{x}^{\prime}_0$ using:
\begin{equation}
    \boldsymbol{x}^{\prime}_{t-1} = \boldsymbol{\mu}^{\prime}_\Theta\left(\boldsymbol{x}^{\prime}_t, t\right) + \sigma^{\prime}_t \epsilon,
\end{equation}
where $\epsilon \sim \mathcal{N}(\mathbf{0}, \boldsymbol{I})$ is random noise independent of $\boldsymbol{x}^{\prime}_t$. Algorithm~\ref{xxxxx} shows the complete sampling procedure of the distilled student model.

\ch{Writing the pseudocode of training and sampling}
\ch{Adding more explanation on the expressions}

\begin{figure}
% \vspace{-1em}
	\centering
	{
            \includegraphics[width=0.5\textwidth]{icml2024/imgs/alg.jpg} }
	\caption{diffusion model distillation}
        \label{fig:methodB}
% \vspace{-1.8em}
\end{figure}

\subsection{Distillation on flexible sub-sequence}
\label{subsec:flexible}

\gill{check}

In the previous derivation, the student extracts the knowledge from a special \gill{unsure which word to use: divisible} sub-sequence $\{\boldsymbol{x}_{ct}\}$ of the teacher where $t \in [1, T^{\prime}]$. Indeed, our proposed method can be extended to a more general case that we distill the knowledge from any given sub-sequence $\{\boldsymbol{x}_{\phi_0},...,\boldsymbol{x}_{\phi_{T^{\prime}}}\}$ of the teacher where $\phi$ is an increasing sub-sequence of $\{0,...,T\}$, $\phi_0 = 0$ and $\phi_{T^{\prime}} = T$. In this general case, the Gaussian mean of $p^{\prime}_\Theta\left(\boldsymbol{x}^{\prime}_{t-1} \mid \boldsymbol{x}^{\prime}_t\right)$ (see Eq.~\ref{eq:pt1t}) is 
\begin{equation*}
\footnotesize
\boldsymbol{\mu}^{\prime}_\Theta\left(\boldsymbol{x}^{\prime}_t, t\right) = \frac{(1-\alpha_{\phi_{t-1}})\sqrt{\alpha_{\phi_{t}}}}{(1-\alpha_{\phi_{t}})\sqrt{\alpha_{\phi_{t-1}}}}\boldsymbol{x}^{\prime}_t + \frac{\alpha_{\phi_{t-1}}-\alpha_{\phi_{t}}}{(1-\alpha_{\phi_{t}})\sqrt{\alpha_{\phi_{t-1}}}}\mathcal{F}_\Theta^{(t)}\left(\boldsymbol{x}^{\prime}_t\right),
\end{equation*}
where $\mathcal{F}_\Theta^{(t)}\left(\boldsymbol{x}^{\prime}_t\right):=\left(\boldsymbol{x}^{\prime}_t-\sqrt{1-\alpha_{\phi_{t}}} \cdot \epsilon^{\prime}_\Theta\left(\boldsymbol{x}^{\prime}_t,t\right)\right) / \sqrt{\alpha_{\phi_t}}$ is a prediction of $\boldsymbol{x}^{\prime}_0$ given $\boldsymbol{x}^{\prime}_t$. Remarkably, $T$ no longer needs to be divisible by $T^{\prime}$. More details of this flexible sub-sequence setting is shown in the Appendix. Such extension is beneficial as it greatly expands the applicability of our distillation under various steps of teacher diffusion models.


% As mentioned in Sec.~\ref{sec:preliminary}, in the existing distillation method on diffusion models. The authors only utilize the intermediate output of the teacher (e.g., the value of hidden variable on each input $x$) to train a student model. However, the value of a hidden variable $v_{t-1}$ is just a instance sampled by $p(v_{t-1}|v_t)$. If we can approximate the teacher's $p(v_{t-1}|v_t)$ on the student model, it is possible to extract the knowledge of the teacher deeply and achieve better performance.

% Our initial idea is that in each round of distillation, we half the number of steps. Then the teacher has $T$ hidden variable $\{v_0, v_1, ..., v_T\}$ and the student has $T/2$ hidden variable $\{v_0, v_2, ..., v_T\}$. To extract underlying knowledge in the conditional distribution of each step, for every two steps of the teacher, we extract its distribution $q(x_t|x_{t-1})$, and let the student mimic it.After many rounds of successive halving, a small student diffusion model with few steps is obtained. 

% Using, the initial idea, multiple rounds are required to obtain a student with a specified number of steps. To address this problem, a improved method is proposed to distill only one round and directly obtain a student with the specified number of steps.

% \subsection{Sucessive-halving}
% \textbf{Lydia: Fill this out}

% \subsection{One-shot Distillation  }
% \textbf{Lydia: Fill this out. Add some discussion on the overhead}





==> sections/methodology_intro.tex <==
\lc{\st{Stress the variable alignment. Stress the importance of  redefining/deriving the forward process of student model, such that the distribution parameters, e.g., mean and standard deviation, can be extracted for training the student. }}

We rethink DDPM-like diffusion models and propose to reduce the number of sampling steps by distilling the knowledge of the teacher model into a student model. Instead of progressive multiple folds, which introduces distortion each fold, \alg utilizes single fold. One crucial challenge is the alignment from the teacher to student hidden variables, as the Markov chain is defined by continuous steps.
\lc{\st{Stress the dfficulty of such single folding - alignment issue.}}
Thus, in this section, we first introduce preliminary of teacher DDPM model, including forward/reverse process definition and training/sampling deployment. After introducing the \gill{unsure which word to use: N times divisible} distillation algorithm \alg, we define the forward and reverse process of the student by matching hidden variables, with regard to the teacher. Then, the training and sampling procedure is designed to deploy the distillation algorithm under the definitions. In addition, we extend the \gill{unsure which word to use: N times divisible}  to flexible sub-sequence to release the constraints on divisible number of teacher steps in distillation.


==> sections/related_work.tex <==
\label{sec:preliminary}
\gill{check:}

\lc{We can skip the first pagraph, as this is not relevant to this paper. Think more carefully what are the relevant related work, corresponding to our contributions} 

Diffusion models, which applies variational inference to derive the general loss for training, are latent variable models for stably generating modern data. Specifically, \cite{sohl2015deep} first generally integrates the forward process for destroying data distribution structure and the reverse process to restore structure in data. It is applicable for various implementations by adapting the hyper-parameters in the forward process and the model architecture or Gaussian distribution parameterization in the reverse process. Tackling with massive variable components, one breakthrough DDPM~\cite{ddpm:ho2020denoising} designs no learnable parameters of the forward process and simplify the Gaussian noise in the reverse process. Thus, DDPM enables stable and effective implementation of diffusion models on high quality image synthesis. The successful implementation of DDPM further advances multiple applications in industry for stability~\cite{ldm:rombach2022high} and scalability~\cite{schuhmann2022laion}, e.g., LDMs~\cite{ldm:rombach2022high} introduces an auto-encoder to map data into a latent
representation with lower dimensions, so as to reduce the model complexity on high resolution image synthesizing scenarios.


 

% \ch{Diffusion models are latent variable models defined by \cite{sohl2015deep}. This paper defines the forward process and reverse process of diffusion models. It applies variational inference to derive the general loss for training diffusion models.}
% \ch{Diffusion model is flexible for various implementations by choosing the hyperparameters in the forward process and the model architecture and Gaussian distribution parameterization of the reverse process. 
% \cite{ho2020denoising} proposes DDPM, which is a commonly used implementation of diffusion models. Many well known diffusion model is based on the basic setting of DDPM. LDMs \cite{rombach2022high} is proposed based on DDPM's model assumpution while introducing a autoencoder to map data $\boldsymbol{x}$ into a latent representation $\boldsymbol{z}$ with lower dimensions, so as to reduce the model complexity on high resolution image synthesizing scenarios. A series of Stable Diffusion models applies LDMs on large-scale datasets \cite{schuhmann2022laion}.}
\lc{More relevant papers will be on reduce the inference/generation overhead of diffusion model }
However, DDPM also suffers from the drawback of slow sampling brought by immense intermediate hidden variables as well as the complex architecture. Predominant Studies nowadays to accelerate the sampling includes three types of methods as follows. One works on fast sampling~\cite{li2023snapfusion, zhao2023mobilediffusion}. Rather than algorithmical simplification, fast sampling facilitates the reverse process by introducing efficient network architecture, i.e., optimizing UNet, is remarkable in mobile accelerations. \cite{li2023snapfusion} proposes an efficient UNet by identifying the redundancy of the original model and reducing the computation, while~\cite{zhao2023mobilediffusion} also comprehensively analyze each component within
the model architecture for further simplification. In summary, fast sampling optimize the inference network structure and can be integrated into other accelerations. Another effort by DDIM~\cite{ddim:conf/iclr/SongME21} focuses on generalizing the Markovian diffusion of DDPM via a family of non-Markovian processes, which is deterministic thus faster. Accordingly, it proposes the novel sampling method to reduce the required number of sampling steps on the trained DDPM model. A noticeable limitation of DDIM is the number of decreased steps. DDIM trades off the number of steps and the quality of generated data, as DDIM sampling approximates a fitting procedure with regard to the number of steps.

Besides, knowledge distillation~\cite{distillation:conf/icml/AsadiDMAB23,distillation:conf/icml/CaoLHRWG23}, which transfers knowledge from a large model to a smaller one, demonstrates superiority for efficient learning tasks. With the significant progress made by knowledge distillation in GANs~\cite{gandistil:conf/cvpr/Cazenavette00EZ23,gandistil:conf/icml/LiuLBL23}, it has also been applied to distill diffusion models. Following the idea of knowledge distillation, progressive distillation~\cite{progress:salimans2022progressive, meng2023distillation}  progressively distill a trained DDIM teacher deterministic
diffusion sampler into  a smaller student diffusion model, so as to enable faster sampling from the student model.\lc{\st{With this reference styles, it's very ugly to start a sentence with citation}} ~\citet{progress:salimans2022progressive} keeps taking half as many sampling steps procedure to the student model, halving the number of required steps each time and distilling down to multiple folds. ~\cite{meng2023distillation} follows the folding optimization and extends to classifier-free guided diffusion implementation of Text-to-Image tasks. Although progressive distillation benefits from efficiency by many halving, each halving process trains a new student model, thus, bringing approximation noise on each folding.


% \ch{DDPM has a slow sampling problem. \cite{li2023snapfusion, zhao2023mobilediffusion} contributes on simplifying the model architecture of the reverse process (This is not on the algorithm side but on the architecture designing side). DDIM \cite{DBLP:conf/iclr/SongME21} proposes a novel sampling method that can reduce the required number of sampling steps on a trained DDPM model.}

% \ch{Briefly introduce model distillation including model distillation on GANs. Model distillation has been applied on diffusion model. Then introduce progressive distillation~\cite{salimans2022progressive, meng2023distillation}}


